VOCALExplore: Pay-as-You-Go Video Data Exploration and Model Building [Technical Report]

We introduce VOCALExplore, a system designed to support users in building domain-specific models over video datasets. VOCALExplore supports interactive labeling sessions and trains models using user-supplied labels. VOCALExplore maximizes model quality by automatically deciding how to select samples based on observed skew in the collected labels. It also selects the optimal video representations to use when training models by casting feature selection as a rising bandit problem. Finally, VOCALExplore implements optimizations to achieve low latency without sacrificing model performance. We demonstrate that VOCALExplore achieves close to the best possible model quality given candidate acquisition functions and feature extractors, and it does so with low visible latency (~1 second per iteration) and no expensive preprocessing.

==> motivatingexample.tex <==
\section{Motivating example} \label{sec:motivatingexample}




\textbf{Deer activity analysis.}
We motivate \system by describing the use case of ecologists we partnered with who study the behavior of deer in the wild~\cite{dellinger:21}. The scientists seek to understand how much time the deer spend on different activities (e.g., eating or traveling).
To study these questions, the ecologists attached GoPro-style cameras to collars on deer. These cameras collected video data for two weeks before the collars automatically released and fell off the deer.

Once the ecologists collected the cameras, they had access to a large quantity of video data (1.4 TB across $800k$ video files) that, were it labeled, would enable them to analyze their research questions.
An ideal solution for these scientists would be to automatically label the videos using a machine learning model.
However, no pretrained model exists for this domain-specific task.
Therefore, the ecologists manually labeled a sample of the videos by tracking annotations in a spreadsheet.
They temporally sampled video clips from the morning, midday, and evening, and performed
their analysis on top of these labeled samples~\cite{dellinger:21}.


This manual labeling process is tedious, and analyzing the labeled samples is limiting, especially when the fraction of labeled data is small.
As an alternative, the scientists could have manually trained a domain-specific model.
This is,
however, challenging for several reasons, especially for users that are not experts in machine learning:
First, it is tedious to search through a large video collection to get samples of
all the different activities that a model needs to learn. While some activities, such as ``foraging'' or ``bedded'' are common, other activities, such as ``looking around'' are rare.
Second, the details of building a model are non-trivial. %
The predominant method today is to fine-tune an existing model~\cite{fei2022searching} because it requires fewer labels than training a deep model from scratch.
While fine-tuning can include performing gradient updates on all layers, for simplicity in this paper we consider just replacing the final, fully connected layer.
The problem is to decide which model to use as a starting point, because embeddings are extracted from this model and used as features for training and inference.
As we show later in the paper, feature selection (which is equivalent to pretrained model selection) significantly impacts model quality.
Coordinating labeling, feature extraction, and model training is also challenging. To achieve high performance, users would need to manually optimize their code, especially to handle incrementally growing sets of features if they want to iteratively perform some labeling and model training before deciding if additional labels are needed, and the required optimizations are nontrivial.





\noindent \textbf{With \system.}
\system addresses these challenges: It supports users in the task of data labeling and model building
by providing an integrated, ``pay-as-you-go'' feature selection and data sampling capability that is both efficient and skew-tolerant, and by offering a task scheduler that minimizes user-visible latencies.







==> outline.tex <==
\section{Introduction}
\begin{itemize}
    \item Video data is dirty and cleaning is hard but important for focusing on interesting bits.
    \item Video data is massive so finding events/environmental conditions of interest is tedious. Generating enough labeled data to train a ML model to automatically do this is tedious.
\end{itemize}

Contributions:
\begin{itemize}
    \item Assist user in identifying and removing unwanted data.
    \item Evaluate different unsupervised feature representations for video data.
    \item Use features and active learning to learn simple domain-specific models.
\end{itemize}

\section{Background}
TBD.

\section{VOCAL-Clean}
\begin{itemize}
    \item Features/models used to identify and remove most dirty data with few manual annotations.
    \item Active learning to prompt user for labels?
    \item \todo{What is novel if we are just using basic features and active learning techniques?} Possible claims to novelty:
    \begin{itemize}
        \item Self-supervised learning and active learning over videos hasn't been studied much. What is and is not possible in this domain?
        \item Can we characterize domains where our approach will work vs. domains where it will not?
        \item Bringing together components into a single system
    \end{itemize}
\end{itemize}

\section{VOCAL-Explore}
\subsection{Features}
\begin{itemize}
    \item Describe basic, pixel-level features.
    \item Describe features extracted from relevant pretrained models.
    \item Describe self-supervised learning over videos.
    \item Discuss tradeoffs between these different feature types and how VOCAL-Explore decides when to use which type.
\end{itemize}

\subsection{Labeling}
\begin{itemize}
    \item Discuss types of user feedback.
    \item Discuss how VOCAL-Explore uses clustering and active learning to incorporate user feedback to generate labeled clusters of video segments.
    \item Discuss how VOCAL-Explore then uses these clusters and labels to train simple domain-specific models.
\end{itemize}

\section{Evaluation}
\subsection{Datasets}
\begin{itemize}
    \item Deer data: Event classification (travel, forage, bedded). Object classification: \todo{??}. Attribute classification (snowy vs. not).
    \item VisualRoad: Event classification (high traffic, low traffic). Object classification: \todo{??}. Attribute classification: \todo{??}.
    \item ActivityNet: Event classification (activity types). Object classification: \todo{??}. Attribute classification: \todo{??}.
\end{itemize}

\subsection{VOCAL-Clean}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/vocal_clean_eval_placeholder.png}
    \caption{Performance of VOCAL-Clean.}
    \label{fig:evalVocalClean}
\end{figure}
\begin{itemize}
    \item Train SVC using pixel-level features: \cref{fig:evalVocalClean}.
    \item Evaluate on different types of dirty data:
    \begin{itemize}
        \item Salt and pepper noise.
        \item \% packet loss.
        \item Obstructed frames (simulate blocked cameras).
    \end{itemize}
\end{itemize}

\subsection{VOCAL-Explore: features}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/vocal_explore_features_perf_eval_placeholder.png}
    \caption{Performance of various features in VOCAL-Explore.}
    \label{fig:evalVocalExploreFeaturesPerf}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/vocal_explore_features_cost_eval_placeholder.png}
    \caption{Cost of extracting of various features in VOCAL-Explore.}
    \label{fig:evalVocalExploreFeaturesCost}
\end{figure}
\begin{itemize}
    \item Train linear classifier on top of features using all labeled data.
    \item Use same categories of models for each dataset (object classification, event classification, …).
    \item Evaluate performance each model type when using different features: \cref{fig:evalVocalExploreFeaturesPerf}.
    \item Evaluate cost (CPU + GPU) of extracting each set of features: \cref{fig:evalVocalExploreFeaturesCost}.
\end{itemize}

\subsection{VOCAL-Explore: labeling}
\begin{figure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/vocal_explore_labeling_eval_placeholder.png}
        \caption{Fixed features.}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/vocal_explore_labeling_eval_placeholder.png}
        \caption{VOCAL-Explore feature selection.}
    \end{subfigure}
    \caption{Performance of VOCAL-Explore.}
    \label{fig:evalVocalExploreLabel}
\end{figure}

\begin{itemize}
    \item Simulate user to generate labeled data for different model types. Train a linear classifier using generated labeled data to measure performance.
    \item Show that VOCAL-Explore performs better than basic strategies, even if user is slightly noisy: \cref{fig:evalVocalExploreLabel}
    \item Each round of computation between user feedback takes on average \todo{XX} seconds, so is fast.
\end{itemize}

Strategies:
\begin{itemize}
    \item Random: each iteration randomly pick $n$ segments to be labeled.
    \item Active learning: each iteration use active learning to pick $n$ segments to be labeled.
    \item Greedy AL: Same as active learning, but also propagate label to top-$k$ most similar segments in feature space.
    \item VOCAL ($sp$, $mp$, $lp$):
    \begin{itemize}
        \item Split cluster if more than $sp$\% do not belong to majority.
        \item Merge two clusters if at least $mp$\% in each cluster belong to same majority ($mp > 0.5$).
        \item Label cluster with majority type if at least $lp$\% belong to majority ($lp > 0.5$).
    \end{itemize}
    \item VOCAL (0, 1, 1): oracle user. Only labels/merges if all are the same. Splits if any are different.
    \item VOCAL (0.1, 0.9, 0.9): noisy user.
\end{itemize}

\section{Related work}

\section{Questions}
\begin{itemize}
    \item \todo{Do we want to tackle how to segment videos, or just stick with a fixed, predetermined segment length?}
\end{itemize}


==> related-work-long.tex <==

\section{Related work -- long}

\subsection{General clustering}

\subsubsection{Efficient Incremental Constrained Clustering~\cite{DBLP:conf/kdd/incrementalconstrained}}
\begin{itemize}
    \item Goal: incrementally add constraints and update clusters without re-running the algorithm. However, optimally updating the clustering is intractable both when adding and removing constraints (when optimizing some objective function). This work identifies conditions where a restricted re-clustering problem can be solved efficiently.
    \item Approach considers must-link constraints ($ML(x, y)$) and cannot-link constraints ($CL(x, y)$).
    \item In most cases the greedy heuristic algorithm only moves the elements involved in the new constraint. \textit{Observation:} It would likely be less work if at each round points similar to $x$ and $y$ were also moved.
    \item Greedy heuristic algorithm that handles cases where a new constraint operates on points that haven't already been constrained, where one of the points is already constrained, or where all of the constraints are must-link constraints, or where the added constraint is a cannot-link. The greedy algorithm fails to efficiently handle the case where a must-link constraint is added on two items that are already constrained. Such an added constraint may cause a large number of cluster reassignments where once the items are assigned to a new cluster, items involved in cannot-link constraints must be reassigned, and this continues recursively.
\end{itemize}

\textit{Problem formalization:}
Optimization objective under constraint addition:
Given a set of points $S$ and set of constraints $C$, let $\Pi$ be a $k$-clustering of $S$ that satisfies all constraints in $C$. Given a new set of constraints $C',\, C \cap C' = \emptyset$, if there exists a $k$-clustering $\Pi'$ that (i) satisfies all constraints in $C \cup C'$ and (ii) $f(\Pi') \leq f(\Pi)$, find the partition $\Pi^*$ that has the minimum $f(\Pi^*)$ from all partitions that satisfy (i) and (ii).

\textit{Evaluation:}
To demonstrate that total re-clustering can significantly alter the cluster membership, after each constraint is added compute the difference between the new clustering and the initial one using the Kullback-Liebler (KL) distance of the mixture distributions each cluster defines.
To evaluate the greedy, incremental algorithm measure how many points are moved from one cluster to another in the incremental case vs. how many points have a changed assignment for the non-incremental case.
Evaluate accuracy by computing cluster purity.

\subsubsection{An Efficient Semi-Supervised Clustering Algorithm with Sequential Constraints~\cite{DBLP:conf/kdd/semisupervisedsequential}}
\begin{itemize}
    \item Goal is to partition data points into clusters while satisfying must-link and cannot-link constraints. Problem formulation allows for some contraints to be violated. It minimizes the cost of violated constraints while ensuring that the clustering is ``good'' (in the sense that similar items are located close together).
    \item Using the assumptions that there are a small number of possible good clusterings and that the eigenvalues of the kernel similarity matrix are skewed, frame the problem as finding the optimal weighted combination of $m$ random clusterings that define the extreme points of a convex hull. This makes the update cost depend on $m$ rather than the number of points.
    \item Generating the $m$ random clusterings is done offline (each time pick a random subset of the features then apply approximate kernel K-means). Use the Hungarian algorithm to realign labels.
    \item Online step: given new pairwise constraints, update the probability simplex vector in $O(p m^2)$, where $p$ is the number of new constraints.
\end{itemize}

\textit{Problem formalization:}
Optimization objective:
\begin{equation*}
\begin{aligned}
\min_{F \in \mathcal{F}} & \sum_{(x_i, x_j) \in \mathcal{M}_t} l_+(F_{i, *}, F_{j, *}) + \sum_{(x_i, x_j) \in \mathcal{C}_t} l_-(F_{i, *}, F_{j, *}) \\
\text{s.t.} \quad & d(F, K) \leq \epsilon
\end{aligned}
\end{equation*}

\textit{Evaluation:}
Evaluate the quality of the clustering based on the normalized mutual information (NMI) between the updated clustering and the ground truth clusters. Compute the average NMI over 10 trials.
They also compute the average time to update the data partitions.

\subsubsection{Semi-Supervised Clustering with User Feedback~\cite{cohn2003semiwithuserfeedback}}
\begin{itemize}
    \item Observe that ``it is easier to criticize than to construct''.
    \item User iteratively provides feedback in the form of constraints that the clustering algorithm uses in future iterations.
    \item Semi-supervised clustering is between unsupervised clustering and supervised learning, where the goal is to learn a mapping from examples to labels that can be used to classify other examples. The goal of semi-supervised clustering is to partition the data into useful clusters with minimal time and effort.
    \item Differences between semi-supervised clustering and active learning (however, authors note that their approach could be considered learning by counterexamples):
        \begin{itemize}
            \item Human selects the data points vs. system picking which points should be labeled next
            \item Human assigns constraints rather than labels
        \end{itemize}
    \item The browsing/annotating process also acts as a process of data exploration and pattern discovery.
    \item They give an example of incorporating incremental constraints into a clustering algorithm for the naive Bayes model of document generation. When incorporating pairwise constraints, learn a weighting variable that specifies the importance of a given term for distinguishing documents. Can use hillclimbing over the gradient of the KL divergence to the mean ($D_{KLM}(x_1, x_2)$) to learn how to adjust the weight to increase or decrease the separation between two documents.
    \item Learning a distance metric becomes part of the clustering algorithm.
    \item Hillclimbing converges to a local minimum of violated constraints.
\end{itemize}

\textit{Problem formalization:}
Probability of document $x$: \\
    $P(x) = \prod_{t_j \in V} P(t_j | \theta) ^{N(t_j, x)}$ \\
Each document is drawn from one of the distributions corresponding to a cluster: \\
    $P(x) = \sum_{i} P(\pi_i) P(x | \pi_i) = \sum_i P(\pi_i) \prod_{t_n \in V} P(t_j | \theta_{\pi_i})^{N(t_j, x)}$ \\
Estimate values for $P(\pi_i)$, $\theta_{\pi_i}$ using EM and then estimate membership by Bayes rule: \\
    $P(\pi_i | x) = P(x | \pi_i) P(\pi_i) / P(x)$ \\
Dissimilarity between documents is proportional to the KL divergence to the meain of their multinomial distributions: \\
    $D_{KLM}(x_1, x_2) = |x_1| D_{KL}(\theta_{x_1}, \theta_{x_1, x_2}) + |x_2| D_{KL}(\theta_{x_2}, \theta_{x_1, x_2})$ \\
To incorporate constraints, augment KL divergence with a weighting function where $\gamma$ represents the importance of term $t_j$ for distinguishing $x_1$ and $x_2$: \\
    $D'_{KL}(\theta_{x_1}, \theta_{x_2}) = \sum_{t_j \in V} \gamma_j \cdot P(t_j | \theta_{x_1})\log \left( \frac{P(t_j | \theta_{x_2})}{P(t_j | \theta_{x_1})} \right)$ \\
Given a constraint that $x_1$ and $x_2$ should be in different clusters, we can compute the gradient to learn which direction to adjust the $\gamma$'s to increase or decrease the separation between two documents: \\
    $\frac{\partial D'_{KLM}(x_1, x_2)}{\partial \gamma_j} = |x_1| P(t_j | \theta_{x_1}) \log \left( \frac{P(t_j | \theta_{x_1 x_2})}{P(t_j | \theta_{x_1})} \right) + |x_2| P(t_j | \theta_{x_2}) \log \left( \frac{P(t_j | \theta_{x_1 x_2})}{P(t_j | \theta_{x_2})} \right) $ \\
Incorporate the $\gamma$'s into the E-step of clustering: \\
    $P(x | \pi_i) = \prod_{t_j \in V} P(t_j | \theta_{\pi_i})^{\gamma_j N(t_j, x)}$ \\

\textit{Evaluation:}
Protocol: Each time clustering converges, add a constraint that two documents should be in different clusters. Then reweight the divergence by a fixed number of hillclimbing steps, re-initialize the cluster prototypes, and repeat the EM training.
Compare between supervised, unsupervised, and semi-supervised learning.
For unsupervised and semi-supervised compute the cluster purity, which is the fraction of data points that would be correctly labeled if all examples were assigned the majority label in each cluster.
For the supervised case, compute the cluster purity in addition to the classification accuracy on an independent test set.

\subsubsection{A probabilistic framework for semi-supervised clustering~\cite{DBLP:conf/kdd/probsemisupervised}}
\begin{itemize}
    \item Framework combines constraint-based and distance-based approaches to clustering methods that incorporate constraints
    \item Introduces an EM-based clustering algorithm called HMRF-KMeans that uses Hidden Markov Random Fields (HMRFs)
    \item HMRF consists of a hidden field, which consists the cluster assignments, $L$, and an observed set, which consists of the data points.
    \item $P(L)$ depends on how many ML/CL constraints are violated. $P(L)$ is higher when fewer constraints are violated
    \item $P(X | L)$ depends on cluster representatives and the distance function
    \item $P(L | X) \alpha P(L) P(X | L)$ therefore incorporates both constraints and distances
    \item Penalizes violated ML constraints more for points that are far apart since that indicates the distance metric is bad (and vice versa for CL constraints)
    \item HMRF-KMeans
    \begin{itemize}
        \item Initialization: find connected components by computing the transitive closure over ML constraints. Then transitively apply CL constraints between connected compmonents. Use these neighborhoods as the initial clusters. If there are more neighborhoods than K, use farthest-first traversal to pick clusters that are far apart and large.
        \item E step: Given the current cluster representatives, assign points to clusters to minimize the objective function. However, actually computing this assignment that minimizes the objective function is intractable. Therefore, use an approximation that greedily sequentially updates the assignment of each point while leaving the rest fixed.
        \item M step: First part: re-compute cluster representatives from their assigned points. This part does not use constraints. Second part: use gradient descent to update each weight according to partial derivative of the objective function with respect to that weight. This step modifies the distance measure to bring similar points closer together and moves dissimimlar points farther apart.
    \end{itemize}
\end{itemize}

\textit{Problem formalization:}
Hidden field $L = \{l_i\}_{i=1}^N$ represents cluster assignments. \\
Observable set of given data points $X = {x_i}_{i=1}^N$, where each random variable is generated from a conditional probability distribution $Pr(x_i | l_i)$. $X$ is conditionally independent given $L$: $Pr(X | L) = \prod_{x_i \in X} Pr(x_i | l_i)$. \\
Probability distribution of the hidden variables obeys $\forall i, Pr(l_i | L - \{l_i\}) = Pr(l_k | \{l_j : l_j \in N_i\})$, where $N_i$ is the set of points that are must-linked or cannot-linked to $x_i$. This means that the probability distribution of $l_i$ only depends on the assignments of neighbors of $x_i$. \\
The probability of a complete label configuration can be expressed as a Gibbs distribution: $Pr(L) = \frac{1}{Z_1} \exp (-V(L)) = \frac{1}{Z_1} \exp \left( - \sum_{N_i \in N} V_{N_i}(L) \right)$, where $V_{N_i}(L)$ expresses the potential for every neighborhood in the configuration. \\
The prior probability of a label configuration is $Pr(L) = \frac{1}{Z_1} \exp (- \sum_i \sum_j V(i, j))$, where $V(i, j)$ is $f_M(x_i, x_j)$ if there is a must-link constraint, $f_C(x_i, x_j)$ if there is a cannot-link constraint, and 0 otherwise. $f_M$ and $f_C$ compute the penalty of violating constraints. \\
The conditional probability of the data given a configuration is $P(X | L) = p(X, \{\mu_h\}_{h=1}^K)$, where $p(X, \{\mu_h\}_{h=1}^K)$ are the cluster representatives. \\
The posterior probability of a cluster label configuration is $Pr(L | X) \propto Pr(L) Pr(X | L)$, so we want to maximize $Pr(L | X ) = \left(\frac{1}{Z_2} \exp \left(-\sum_i \sum_j V(i, j) \right) \right) \cdot p(X, \{\mu_h\}_{h=1}^K)$ \\
The objective function is to miniimize the posterior energy of the HMRF: \\
\begin{equation*}
    \begin{aligned}
        J_{obj} &= \sum_{x_i \in X} D(x_i, \mu_{l_i}) + \sum_{(x_i, x_j) \in M} w_{ij} \psi_D(x_i, x_j) \mathbbm{1}[l_i \neq l_j] \\
            &+ \sum_{(x_i, x_j) \in C} \bar{w}_{ij} (\psi_{D \max} - \psi_D(x_i, x_j)) \mathbbm{1}[l_i =l_j] + logZ
    \end{aligned}
\end{equation*}
where $w$ is the cost of violating a constraint, and $\psi_D$ is a penalty scaling function that scales with the distance between two points. Violated must-link constraints have a higher penalty when the points are far apart, and vice versa for violated cannot-link constraints.

\subsubsection{Integrating constraints and metric learning in semi-supervised clustering~\cite{DBLP:conf/icml/mpckmeans}}
\begin{itemize}
    \item Incorporates both constraints and distance-learning methods into an algorithm called MPCK-Means
    \item Constraint-based approaches modify the clustering algorithm objective function so that it includes the satisfaction of constraints
    \item Metric-based approaches train the distance metric to satisfy the constraints
    \item The objective function for k-means with constraints is
\end{itemize}
\begin{equation*}
    \begin{aligned}
        \mathcal{J}_{pckmeans} &= \sum_{x_i \in X} \|x_i - \mu_{l_i} \|^2 + \sum_{(x_i, x_j) \in M} w_{ij} \mathbbm{1}[l_i \neq l_j] \\
            &+ \sum_{(x_i, x_j \in C)} \bar{w}_{ij} \mathbbm{1}[l_i = l_j]
    \end{aligned}
\end{equation*}
\begin{itemize}
    \item In K-means with metric learning, Euclidean distance is parametrized. This enables each dimension to be scaled by a different weight, or possibly create new features that are combinations of existing ones.
    \item Parametrized distance: $\| x_i - x_j \| _A = \sqrt{(x_i - \mu_{l_i})^T A (x_i - \mu_{l_i})}$
    \item Its objective function is
\end{itemize}
\begin{equation*}
    \begin{aligned}
        \mathcal{J}_{mkmeans} = \sum_{x_i \in X} \left( \| x_i - \mu_{l_i}\| ^2 _{A_{l_i}} - \log (\det (A_{l_i})) \right)
    \end{aligned}
\end{equation*}
\begin{itemize}
    \item Combine the two objective functions by replacing the distance term of kmeans:
\end{itemize}
\begin{equation*}
    \begin{aligned}
        \mathcal{J}_{combined} &= \sum_{x_i \in X} \left( \| x_i - \mu_{l_i}\| ^2 _{A_{l_i}} - \log (\det (A_{l_i})) \right) \\
            &+ \sum_{(x_i, x_j) \in M} w_{ij} \mathbbm{1}[l_i \neq l_j] + \sum_{(x_i, x_j) \in C} \bar{w}_{ij} \mathbbm{1}[l_i = l_j]
    \end{aligned}
\end{equation*}
\begin{itemize}
    \item Scale the cost of violating constraints by the distance between them (ML constraint violation penalty should be higher for points that are far apart and vice versa for CL constraints): $f_M (x_i, x_j) = \frac{1}{2}\|x_i - x_j\|^2_{A_{l_i}} + \frac{1}{2} \| x_i - x_j \|^2_{A_{l_j}}$.
    \item When these scaling functions are incorporated into the combined objective function it becomes:
\end{itemize}
\begin{equation*}
    \begin{aligned}
        \mathcal{J}_{mpckm} &= \sum_{x_i \in X} \left( \| x_i - \mu_{l_i}\| ^2 _{A_{l_i}} - \log (\det (A_{l_i})) \right) \\
            &+ \sum_{(x_i, x_j) \in M} f_M(x_i, x_j) \mathbbm{1}[l_i \neq l_j] \\
            &+ \sum_{(x_i, x_j) \in C} f_C(x_i, x_j) \mathbbm{1}[l_i = l_j]
    \end{aligned}
\end{equation*}
\begin{itemize}
    \item Initialization step seems the same as in HMRF-KMeans
    \item E-step: Randomize order of points and then assign each to the cluster that minimizes the combined cost of distance to the center and constraint violations. At the end of this step $\mathcal{J}_{mpckm}$ will be smaller or the same.
    \item M-step part 1: Re-estimate cluster centroids (doesn't require constraints)
    \item M-step part 2: perform metric learning by adjusting matrix $A$ for each cluster. To get the updated weights, take the partial derivative $\frac{\partial \mathcal{J}_{mpckm}}{\partial A_h}$ and set it to zero. The closed-form solution requires taking the inverse of each $A_h$ which is expensive, so use a diagonal matrix which has a cheaper solution.
    \item The paper gives the closed form solution to compute the d'th diagonal element of the h-th cluster metric, $a_{dd}^{(h)}$. It scales the weight of each feature relative to its contribution to the overall cluster dispersion, and stretches each dimension in an attempt to fix constraint violations.
    \item It's possible to use a single metric or different ones for each cluster.
    \item Evaluate by computing the F-measure with 5-fold cross-validation.
\end{itemize}

\subsubsection{Active learning of constraints for semi-supervised clustering~\cite{DBLP:journals/tkde/alsemisupervised}}
\begin{itemize}
    \item Pick which points to ask about by balancing the uncertainty of each data point with the expected number of queries required to resolve the uncertainty
    \item \textit{Neighborhood}: set of points known to belong to the same cluster. Different neighborhoods have cannot-link constraints between them
    \item \textit{Uncertainty}: probability the point belongs to different known neighborhoods
    \item When estimating the neighborhood assignment of a point, only consider the labeled instances to be robust to bad clusterings
    \item To compute the similarity between instances, train a random forest using the current clustering assignments as labels. Then measure the number of times the two instances end up in the same leaf in each tree.
    \item Probability of a point belonging to a neighborhood is proportional to the average similarity to all points in that neighborhood. Uncertainty is the entropy of neighborhood membership.
    \item Expected number of queries to get a must-link constraint for a new point can be computed using the probability the point belongs to each neighborhood. Ask the user in descending order of probabilities.
    \item Pick the instance that maximizes the ratio between the gain of information vs. the expected number of queries.
\end{itemize}

\textit{Problem formalization:}

Current clustering assignment: $\pi$ \\
Current set of neighborhoods: $\mathcal{N} = \{N_1, \ldots, N_l \}$ \\
Goal is to estimate $p(x \in N_i)$ for each data point $x \in D$ and neighborhood $i \in \{1, \ldots l\}$ \\
The similarity between $x_i$ and $x_j$ is given by $M(x_i, x_j)$ \\
The probability of a point belonging to a neighbhood is proportional to the average similarity between $x$ and the elements in $N_i$:
\begin{equation*}
    \begin{aligned}
        p(x \in N_i) = \frac{\frac{1}{|N_i|} \sum_{x_j \in N_i} M(x, x_j)}{\sum_{p=1}^l \frac{1}{|N_p|} \sum_{x_j \in N_p} M(x, x_j)}
    \end{aligned}
\end{equation*}
Entropy of neighborhood membership. Higher $H$ means the point is more uncertain. $H(\mathcal{N} | x) = -\sum_{i=1}^l p(x \in N_i) \log_2 p(x \in N_i)$ \\
Expected number of queries to learn the membership of $x$: $\mathbb{E}[q(x)] = \sum_{i=1}^l i \cdot p(x \in N_i)$ \\
Ask next about the instance that maximizes: $x^* = \arg\max_{x \in U} \frac{H(\mathcal{N} | x)}{\mathbb{E}[q(x)]}$, where $U$ is the set of unconstrained points. \\

\subsubsection{Constraint-based clustering selection~\cite{DBLP:journals/ml/constraintselection}}
\begin{itemize}
    \item Introduce a technique called COBS (constraint-based selection)
    \item Propose that choosing the right algorithm and hyperparameter values is more important than modifying one algorithm to consider constraints. Intuition: different clustering algorithms have different biases and no one performs best on all clustering problems.
    \item Approach: generate a set of clusterings using several unsupervised algorithms and hyperparameter values (generated using grid search). Then, pick the one that satisfies the most constraints.
    \item Find this approach outperforms semi-supervised methods (MPCKMeans, FOSC-OpticsDend, COSC (based on spectral clustering))
\end{itemize}

\subsubsection{Scalable Active Temporal Constrained Clustering~\cite{DBLP:conf/edbt/activetemporalclustering}}
\begin{itemize}
    \item Iteratively select the most informative pairs of objects. Technique is called ``border''.
    \item Key idea: select a small set of objects at cluster borders and query about the most uncertain pairs.
    \item Extra optimization: Add inferred constraints based on nearest nighbors to increase the total number of constraints.
    \item Approach extends the CVQE clustering algorithm.
    \item Steps:
    \begin{enumerate}
        \item Pick points with highest border score for each cluster.
        \item Estimate the uncertainty of each of these points. When uncertainty is high, a point is in areas with mixed class labels and many violated constraints.
        \item Split selected objects into two sets: for all $(x, y) \in X: label(x) = label(y)$, and for all $(p, q) \in Y: label(p) \neq label(q)$. From $X$, pick the pairs that are most likely to belong to different clusters. From $Y$ pick the points that are most likely to belong to the same cluster.
    \end{enumerate}
    \item To add inferred constraints given constraint $(p, q, w_{pq})$, add $(a, b, w_{ab})$ for all $a \in \mu nn(p)$ and $b \in \mu nn(q)$, where $w_{ab}$ is $w_{pq}$ scaled by triangle kernel functions that measure the influence of $p$ and $q$ on $a$ and $b$ respectively.
\end{itemize}

Key metrics: \\
Border score of item $a$: $bor(a) = \frac{(a - c_i)^2}{(a - c_{\psi(i)})^2 (1 + ml(a)) (1 + cl(a))}$, where $ml(a)$ and $cl(a)$ are the sums of weights of constraints of $a$. By including them, in the denominator, the approach favors objects that have fewer constraints to increase the diversity of points in the constraint set. \\
Uncertainty score of item $a$: $sco(a) = ent(\mu nn(a)) + \frac{vl(ml(a)) + vl(cl(a))}{ml(a) + cl(a) + 1}$. $ent(\mu nn(a))$ is the entropy of class labels of the $\mu$ nearest neighbors of $a$. $vl(ml(a))$ and $vl(cl(a))$ are the sums of violated constraints of a. \\
For points in $X$ (in the same cluster), a \textit{high} $val$ means points are more likely to belong to different clusters.
$$
    val(x, y) = \frac{(x-y)^2 (1 + sco(x)) (1 + sco(y))}{(1 + ml(x) + cl(x)) (1 + ml(y) + cl(y))}
$$
For points in $Y$ (in different clusters), a \textit{low} $val$ means points are more likely to belong to the same cluster.
$$
    val(p, q) = \frac{(p-q)^2 (1 + ml(p) + cl(p)) (1 + ml(q) + cl(q))}{(1 + sco(p)) (1 + sco(q))}
$$

\subsubsection{Bayesian Active Clustering with Pairwise Constraints~\cite{DBLP:conf/pkdd/bayesiaanactiveclustering}}
\begin{itemize}
    \item Select the most informative pair of points considering uncertainty and martinal information gain.
    \item Bayesian clustering model models conditional probability of cluster assignments given data points. It uses a prior that encourages large separations between clusters.
    \item Approach: each iteratoin, pick a pair from unlabeled pairs considering two measures.
    \begin{itemize}
        \item Variables: instance $x_i$, model parameter $W$, pair label $z_{a, b}$, all constraints $Z$, data-dependent prior $P(W | X, \theta)$ with parameter $\theta$
        \item Uncertainty: pick pair with largest marginal entropy of the pair label.
        $$(x_a^t, x_b^t) = \arg\max_{(x_a, x_b) \in U^t} H(z_{a, b} | Z_{t-1}, X, \theta)$$
        \item Info: pick pair with the largest marginal information gain (maximize entropy reduction):
        $$(x_a^t, x_b^t) = \arg \max_{(x_a, x_b) \in U^t} H(Z_{a, b} | Z_{t-1}, X, \theta) - H(Z_{a, b} | W, Z_{t-1}, X, \theta)$$
    \end{itemize}
    \item Uncertainty metric tries to reduce the uncertainty of the pair label. Info objective aims to reduce the model uncertainty.
\end{itemize}

\subsubsection{Distance Metric Learning, with Application to Clustering with Side-Information~\cite{DBLP:conf/nips/distancemetriclearning}}
\begin{itemize}
    \item Goal: given sets of similar and dissimilar pairs of points, learn a distance metric that satisfies those relationships
    \item Compared with prior work on multidimensional scaling (MDS) and locally linear embedding (LLE) metric learning learns a full metric over the full input space rather than being constrained to the training dataset
    \item Learned distance metric parametrizes distance with a PSD matrix $A$ that parametrizes the family of Mahalanobis distances: $d(x, y) = d_A(x, y) = \| x - y \|_A = \sqrt{(x - y)^T A (x - y)}$
    \item Convex optimization problem minimizes the squared distances between similar points while requiring that dissimilar points aren't the same (so that the dataset isn't collapsed to a single point).
    \item If $A$ is diagonal, can solve the optimization problem efficiently using Newton Raphson method
    \item Otherwise, use gradient descent with some special care to make sure $A$ stays PSD
\end{itemize}

\textit{Problem formalization:}

Optimization problem:
\begin{mini*}|s|
    {A} {\sum_{(x_i, x_j) \in \mathcal{S}} \|x_i - x_j \|_A^2}
    {}{}
    \addConstraint{\sum_{(x_i, x_j)\in \mathcal{D}} \| x_i - x_j \|_A}{\geq 1}
    \addConstraint{A}{\succeq 0}
\end{mini*}

\subsubsection{Temporal subspace clustering for
human motion segmentation~\cite{DBLP:conf/iccv/temporalhumanmotion}}
\begin{itemize}
    \item Temporal subspace clustering (TSC) uses temporal regularization to encode sequential relationships and jointly learns representation codings and the associated dictionary (i.e., given $X \approx D Z$, learn $D$ and $Z$). Then the codings are used to construct an affinity graph and group temporal segments via spectral clustering
    \item The goal of TSC is to first group the $n$ samples into $m,\, (m \geq k)$ sequential segments, and then cluster the $m$ segments into $k$ subspaces
    \item For normal subspace clustering the frobenius norm of the coefficient matrix $Z$ is a good regularizer because it enforces the block diagonal structure of $Z$
    \item Temporal regularizer $f(Z)$ encodes that adjacent columns (data points) should be similar
    \item After learning $Z$ and $D$, use $Z$ to construct an affinity graph then apply the normalized cuts clustering algorithm to find the subspaces. The similarity measurement to construct the graph uses the fact that sequential neighbors are highly correlated: $G(i, j) = \frac{z_i^{\mathsf{T}}z_j}{\|z_i\|_2 \|z_j\|_2}$
\end{itemize}

\textit{Problem formalization:}

Objective function:
\begin{mini*}[s]
    {Z, D}{\| X - DZ \|_{\textnormal{F}}^2 + \lambda_1 \|Z\|_{\textnormal{F}}^2 + \lambda_2 f(Z)}
    {}{}
    \addConstraint{Z}{\geq 0}
    \addConstraint{D}{\geq 0}
    \addConstraint{\|d_i\|_2^2}{\leq 1, \quad}{i = 1, \ldots, r}
\end{mini*}
where $\|Z\|_{\textnormal{F}}^2 = \sum_{i = 1}^r \sum_{j=1}^n Z_{ij}^2$ ($r$ is the number of bases in the dictionary).
The first two constraints say the dictionary and coding matrix should be non-negative, and the last one controls the model complexity.
The temporal Laplacian regularizer is defined as:
\begin{equation*}
    f(Z) = \frac{1}{2} \sum_{i=1}^n \sum_{j=1}^n w_{ij} \|z_i - z_j\|_2^2 = \Tr\left(Z L_T Z^{\mathsf{T}}\right)
\end{equation*}
$L_T = \tilde{D} - W$ is a temporal Laplacian, where $\tilde{D}_{ii} = \sum_{j=1}^n w_{ij}$, and $W$ is the weight matrix capturing sequential relationships in $X$. If $s$ is the number of neighbors for each sample, then
\begin{equation*}
    w_{ij} =
    \begin{cases}
        1, \quad \textnormal{if } |i-j|\leq \frac{s}{2} \\
        0, \quad \textnormal{otherwise.}
    \end{cases}
\end{equation*}
so neighbors of $x$, $\{x_{i-s/2}, \ldots, x_{i+s/2}\}$ are encouraged to have the same codings $\{z_{i-s/2}, \ldots, z_{i+s/2}\}$.

\subsection{Image clustering}

\subsubsection{QCluster~\cite{DBLP:/conf/sigmod/qcluster}}
\begin{itemize}
    \item Incrementally learn a clustering to return images relevant to a query. Recognizes the challenge posed by the gap between high-level concepts and low-level features.
    \item Rather than finding a single cluster that represents a query, enable a query to be represented by multiple clusters.
    \item Approach: Given a query consisting of one or more images, query to find nearby images. The user assigns relevance scores to each returned item. Based on these relevance scores, assign each relevant image to an existing cluster, or create a new one. Then merge similar clusters to reduce the total number of clusters. Finally, use the cluster representatives from the new clustering as input for the next round of query/feedback.
    \item Qcluster uses a quadratic distance function so that clusters don't have to be spherical and each dimension can be assigned a different weight.
    \item To get the initial clustering, it uses a higherarchical clustering algorithm where each point is originally in its own cluster. They then compute descriptive statistics about each cluster (mean, covariance, radius). To determine the radius, they assume the data follows a Gaussian distribution and adjust the radius based on the significance level.
    \item Classification stage: first find the cluster that maximizes the posterior probability that the item came from that cluster given the item was observed. Key idea is to assign a point to the nearest cluster. However, if the closest cluster is farther away than its radius, the item is placed into a new clustr.
    \item To find clusters to merge, use Hotelling's $\textnormal{T}^2$ to decide whether two clusters represent the same population. This assumes the clusters follow normal distributions and have the same covariance. If clusters are merged, characterize the combined cluster by combinations of the sub-cluster's mean, covariance, and weight.
\end{itemize}

\textit{Problem formalization:}
At the classification stage, maximize the posterior probability $P(C_k, | x)$:
\begin{equation*}
    \begin{aligned}
        P(C_k | x) &= \frac{w_k f_k(x)}{\sum_{i=1}^g w_i f_i(x)} \\
            &= \frac{(prior_k) \times (likelihood_k)}{\sum \left[ (prior_k) \times (likelihood_k) \right]} \text{ for } i=1, \ldots, g
    \end{aligned}
\end{equation*}
where $f_i$ is the pdf of cluster $C_i$.

\textit{Evaluation:}
Procedure: generate 100 random initial queries and evaluate the retrieval quality for 5 feedback iterations. Results are averaged over the 100 queries. To evaluate the efficiency, they measure the CPU cost of various approaches. To measure the quality, they plot the precision and recall using the ground-truth categorical information as the number of returned images varies. They also compute the error rate as $1 - C/N$, where $N$ is the total number of elements, and $C$ is the number of elements that are correctly classified to their original cluster after removing each point from its final cluster and then re-assigning it to a cluster following the classification procedure.

\subsubsection{Active image clustering: seeking constraints from humans to complement algorithms~\cite{DBLP:conf/cvpr/imageconstraintsfromhumans}}
\begin{itemize}
    \item Proposed algorithm: Cluster objects using both constraints and distances. Ask a person about two objects. Repeat.
    \item Assumes that a distance matrix is provided.
    \item To estimate the probability that a data pair belongs to the same cluster, use consensus clustering to produce multiple clusterings using KMeans with random initial centroids.
    \item Strategy for picking which objects should be labeled: pick objects where the answer may have a large effect on the way objects are clustered (maximize the product of the probability the answer will cause a change in the current clustering and the size of the change).
    \item Perform clustering using minimum spanning forests (MSFs) that is similar to bottom-up hierarhical clustering.
    \item Propose some heuristics based on the observation since most constraints minimally affect the clustering. However, it's possible that changes have domino effects (e.g., adding a must-link constraint to data points that have a cannot-link constraint between their clusters).
    \item Apparently complete algorithm is too complex to include in the paper.
\end{itemize}

\textit{Problem formalization:}
Each round ask the user about the pair $(\hat{d}_i, \hat{d}_j) = \arg\max_{d_i, d_j} E_J (d_i, d_j)$, where $E_J (d_i, d_j)$ is the expected change in the Relative Jaccard's Coefficient (RJC). The Relative Jaccard's Coefficient of clustering $C_2$ w.r.t. $C_1$ is $JCC_{C_1}(C_2) = \frac{SS}{SS + SD + DS}$, where $SS$ is the number of pairs that are in the same cluster in both $C_1$ and $C_2$, $SD$ is the number of pairs that are in the same cluster in $C_1$ but are in different clusters in $C_2$, and $DS$ is the number of pairs that are in different clusters in $C_1$ but in the same cluster in $C_2$.
\begin{equation*}
    \begin{aligned}
        E_J(d_i, d_j) &= |JCC_{H_q}(H_q) - ( P(d_i, d_j)J_{q+1}^{d_i, d_j, y} + \\
            & (1 - P(d_i, d_j))J_{q+1}^{d_i, d_j, n})|
    \end{aligned}
\end{equation*}
where $JCC_{H_q}(H_q) = 1$, $P(d_i, d_j)$ is the probability of $d_i$ and $d_j$ being in the ame cluster, $J_{q+1}^{d_i, d_j, y}$ is the RJC of a clustering after $q+1$ questions w.r.t. $H_q$ if the new constraint is $d_i$ and $d_j$ belong to the same cluster. $J_{q+1}^{d_i, d_j, n}$ is equivalent for the case where the $(q+1)$-th constraint is they are in different clusters.

\textit{Evaluation:}
Plot the Jaccard's Coefficient relative to ground truth as the number of quesions increases.

\subsubsection{Iterative Human and Automated Identification of Wildlife Images}

\subsection{Video clustering}

\subsubsection{Subspace clustering for sequential data~\cite{DBLP:conf/cvpr/subspacesequential}}
\begin{itemize}
    \item Subspace clustering: Assume the data lies in a union of lower-dimensional subspaces. Cluster the data according to their subspaces.
    \item Incorporate a neighbor penalty term to encode similarity between sequential data points.
    \item Useful for video scene segmentation and face clustering.
    \item Background: Given a matrix of samples $X = [x_1, \ldots, x_N] \in \mathbb{R}^{D \times N}$, each data point can be represented by a linear combination elements in a dictionary $A = [a_1, \ldots, a_n] \in \mathbb{R}^{D \times n}$: $X = AZ$, $Z = [z_1, \ldots, z_N] \in \mathbb{R}^{n \times N}$ is the coefficient matrix. However, if the dictionary is unknown the data samples can be used as the dictionary : $A = X$. When this happens, $z_{ij}$ represents the similarity of point $x_i$ to $x_j$.
    \item Propose an algorithm that computes the number of clusters so it doesn't have to be specified in some cases.
\end{itemize}

\textit{Problem formalization:}
Objective function:
\begin{equation*}
    \begin{aligned}
        \min_{\mathbf{Z}, \mathbf{E}} \frac{1}{2} \| \mathbf{E} \|_F^2 + \lambda_1 \| \mathbf{Z} \|_1 + \lambda_2 \| \mathbf{Z} \mathbf{R} \|_{1, 2} \\
        \text{s.t. } \quad \mathbf{X} = \mathbf{X} \mathbf{Z} + \mathbf{E}
    \end{aligned}
\end{equation*}
where $\mathbf{E}$ is Gaussian noise. The penalty term $\|\mathbf{Z} \mathbf{R}\|_{1, 2}$ enforces column similarity

\textit{Evaluation:}
Compute subspace clustering error (SCE):
\begin{equation*}
    \text{SCE} = \frac{\text{num. misclassified points}}{\text{total num. points}}
\end{equation*}
Report minimum, maximum, median, and mean on clustering error.

\subsubsection{Cottontail DB: an open source database system for multimedia retrieval and analysis~\cite{DBLP:conf/mm/cottontaildb}}
\begin{itemize}
    \item Stores both feature vectors along with other metadata like textual descriptors
    \item Supports both boolean queries and nearest neighbor search
    \item For NN search, uses LSH-based indexes, and for boolean search uses hash-based indexes
    \item Uses column storage to read only necessary information from disk and parallelizes processing via chunking
\end{itemize}

\subsubsection{Cineast: a multi-feature sketch-based video retrieval engine~\cite{DBLP:conf/ism/cineast}}
\begin{itemize}
    \item Target use case is known item search: find a specific video
    \item Supports searching for a particular video clip based on edge or color sketches, or sample video sequences
    \item Features are derived from low-level features like pixels, audio, subtitle text
    \item Performs a similarity search per-feature and then computes a linear combination of the per-feature scores
    \item Offline phase: perform feature extraction and indexing
    \item Online phase: retrieve
    \item Uses color histograms to decide where to split videos into shots
    \item User is responsible for specifying which features to use and how to weight them when computing the combined score
\end{itemize}


\subsubsection{Vitrivr-Explore: guided multimedia collection exploration for ad-hoc video search~\cite{DBLP:conf/sisap/vitrivrexplore}}
\begin{itemize}
    \item Target use-case: user wants to see similar video clips to some example
    \item Supports relevance feedback-driven exploration using self-organizing maps
    \item In addition to low-level features like color and motion, extract features from MobileNet V1 on the momst representative frame per shot
    \item Relevance feedback process:
    \begin{itemize}
        \item User marks each segment as positive or negative, or abstains from marking that segment
        \item Based on these labels, generate traiing data for the SOM by sampling $k$ elements per positively marked segment and $k'$ elements per negatively marked segment using NN search
    \end{itemize}
    \item The paper does not say whether the training is incremental or how to pick which features to train on
\end{itemize}

\subsubsection{Real-time large scale near-duplicate web video retrieval~\cite{DBLP:conf/mm/nearduplicateweb}}
\begin{itemize}
    \item Generate spatiotemporal features based on gray intensity distribution and temporal behavior across frames. Also prooses an index based on inverted files that enables fast histogram intersection to find duplicates
    \item To generate the spatiotemporal feature:
    \begin{itemize}
        \item Sample one frame per second and compute the ordinal measure (an image correspondence feature) by splitting it into a $3 {\times} 3$ grid and computing the average gray level in each cell. Then sort the intensities and assign a rank to each cell
        \item Then compute pairwise ordinal relations between blocks and express this as a binary vector $A$ where $|A| = C_{numblocks}^2$
        \item Then use feature selection to get a smaller set of features (they use an entropy-based process to pick the $K$ most informative features)
        \item Finally, use w-shingling ($w=2$) to generate temporal features. Each token is a $K$-dimensional binary vector, so there are $2^{2\cdot K}$ tokens in the vocabulary
        \item Represent the original video using a histogram of the visula shingles (bag of visual shingles, BoVS)
    \end{itemize}
\end{itemize}

\subsubsection{Near-duplicate video retrieval with deep metric learning~\cite{DBLP:conf/iccvw/nearduplicatedeepmetric}}
\begin{itemize}
    \item To evaluate similarity, uses deep metric learning (DML) with features extracted from intermediate layers of CNNs to learn an embedding
    \item Train DML model using triplets (anchor, a positve sample in the same class as the anchor, and a negative sample in a different class)
    \item Definition of near-duplicate: same content, but different in photometric properties (e.g., lighting), editing ooperations (e.g., watermark), encoding parameters, file format, length, …
    \item The method is dataset independent, so it can be trained and used on different datasets
    \item Per-frame descriptors: use Maximmum Activation of Convolutions (MAC): extract features from each layer and use max-pooling to condense to a single value per channel, concatenate them, then normalize. The paper uses AlexNet (~1300 dimensions) and GoogleNet (~5500 dimensions).
    \item To go fromm frame-level descriptors to global video descriptors, uniformly sample $n$ frames/second, then average and normalize the frame descriptors
    \item The similarity between videos is computed as the squared Euclidean distance in embedding space
    \item Training assumes that near-duplicate video relationships are known
    \item Possible methods for siilarity computation across frames:
    \begin{itemize}
        \item Early fusion: average/normalize frame descriptors before forward propagation. This is computationally less expensive.
        \item Late fusion: feed every frame descriptor into network, then average/normalize the outputs to get the embedding. This is more expensive but performs better.
    \end{itemize}
\end{itemize}

\subsubsection{Constrained Clustering and Its Application to Face Clustering in Videos~\cite{DBLP:conf/cvpr/faceclustering}}
\begin{itemize}
    \item Problem statement: given the number of people ($K$), detected faces and associated tracks, and features of each face, partition all faces into $K$ clusters
    \item In contrast to clustering faces in images, when they appear in a video there is additional knowledge of their temporal and spatial tracks
    \item These constraints are incorporated into a clustering model based on Hidden Markov Random Fields (HMRF)
    \item The temporal tracks of faces generate must-link and cannot-link constraints. The weights of these constraints can be learned
    \item Additional smoothness constraints are enforced:
    \begin{itemize}
        \item If two observations are similar, then their labels should be similar
        \item If there is a must-link/cannot-link constraint between $x_1$ and $x_2$, and $x_2$ is close to $x_3$, then there is a must-link/cannot-link constraint between $x_1$ and $x_3$
    \end{itemize}
    \item Model is optimized using the simulated field algorithm to learn the model parameters and wieghts of constraints (when working on a particular latent variable, fix the states of its neighbors) because computing the exact solution is intractable
    \item
    \item Proposed algorithm has high complexity, but a faster heuristic first clusters a subset of faces (sampled from all tracks) and then propagates the labels to the rest of the faces in each track
    \item A combined pairwise potential function penalizes configurations that violate either propagated constraints or label-level local smoothness. One constant determines how far labels propagate for smoothness, and another determines the tradeoff between satisfying constraints and smoothness
\end{itemize}

\subsubsection{Collaborative deep metric learning for video understanding~\cite{DBLP:conf/kdd/deepmetricunderstanding}}
\begin{itemize}
    \item Goal is to unify various tasks over videos into one framework
    \item Embed videos based on audio and visual content into a latent space that preserves video-to-video relationships
    \item This embedding network can be used in multiple downstream tasks like classification and recommendation
    \item This approach assumes a similarity graph (nodes = videos, edges = videos are similar) is given
    \item Train the model using triplet loss
\end{itemize}

\subsubsection{Fast unsupervised ego-action learning for first-person sports video~\cite{DBLP:conf/cvpr/egoactionsports}}
\begin{itemize}
    \item Use unsupervised learning on top of motion histograms to cluster videos
    \item Use a stacked Dirichlet process mixture model: the first DPM learns the motion codebook, and the second DPM learns the action categories
    \item Measure motion using sparse optical flow vectors, and for robustness only keep those that are consistent according to RANSAC, then aggregate into a normalized motion histogram
    \item Identify two types of important motion: periodic (frequency component) and instantaneous (directional component)
    \item The directional component is encoded in a histogram with 36 bins (combination of direction, magnitude, and direction), and frequency component is encoded in a 16 bin histogram (8 for each X and Y) after computing DFT over the average flow magnitude with a 64 frame sliding window
\end{itemize}

\subsection{Self-supervised learning}

\subsubsection{A simple framework for contrastive learning of visual representations~\cite{DBLP:conf/icml/SimCLR}}
\begin{itemize}
    \item SimCLR: learn good embeddings by maximizing the agreement between different augmented views of the same data example
    \item Types of augmentations for images: random cropping + resize, color distortion, Gaussian blur
    \item Use other augmented views within a mini batch as negative examples. Using larger batch sizes leads to better performance because there are more negative examples within a batch.
\end{itemize}

\subsubsection{Bootstrap your own latent: a new approach to self-supervised learning~\cite{DBLP:conf/nips/byol}}
\begin{itemize}
    \item Learns good embeddings without needing negative examples
    \item Uses a paired network: an online model (that is eventually used to produce embeddings), and a target network whose weights are a moving average of the online one. Given an augmented image, the online network tries to predict the target network's representation of a different augmented view of the same image.
    \item Find this approach is more robust to augmentation operations than contrastive methods.
    \item Uses the same image augmentations as SimCLR (random patch + resize with horizontal flip, color distortion, Gaussian blur)
\end{itemize}

\subsubsection{Spatiotemporal contrastive video representation learning~\cite{DBLP:conf/cvpr/stcontrastivevideo}}
\begin{itemize}
    \item Contrastive learning goal: two augmented clips from the same video have similar embeddings while those from different videos are pushed away
    \item Both spatial and temporal augmentations are important for videos (22\% improvement in accuracy when using both types vs. one or the other)
    \item Temporal augmentation: sample shorter clips within the video. With higher probability, sample clips that are close in time to reduce the difference in content. (Note, this is different than the finding in \cite{DBLP:conf/cvpr/largestudystlearning} that found large temporal gaps between clips (~1min) benefited performance.)
    \item Spatial augmentation: apply the same augmentation operations to each frame within a clip to maintain temporal relationships
    \item Use a 3D-ResNet-50 backbone, and end up with a 2048-D vector
    \item For pre-training, each clip contains 16 frames sampled with a temporal stride of 2 (e.g., every other frame). For evaluation, use a single 32 frame clip sampled with a temporal stride of 2.
\end{itemize}

\subsubsection{Multiview pseudo-labeling for semi-supervised learning from video~\cite{DBLP:journals/corr/multiviewvideo}}
\begin{itemize}
    \item RGB, optical flow, and temporal difference are used as different representations of the same video clip. The same augmentations are applied to each frame within a clip for consistency (flip, crop, color, rotation, translation, etc.).
    \item Optical flow and temporal difference are converted to a pixel-like representation so they can be fed into the same network
    \item Use 3D-ResNet-50 with 8-frame clips sampled with stride 8 with input size $224 {\times} 224$
    \item For evaluation, uniformly sample 10 clips from the video and average the scores
\end{itemize}

\subsubsection{Long-short temporal contrastive learning of video transformers~\cite{DBLP:journals/corr/longshortvideo}}
\begin{itemize}
    \item Goal: learn useful embeddings by learning to predict the representation of a longer clip from a shorter one
    \item Long clips are 8 seconds long, and short clips are 2 seconds long. Both contain the same number of frames, just sampled at different frame rates.
    \item Negative examples: clips extracted from different videos
    \item Use the same data augmentations as \cite{DBLP:conf/cvpr/largestudystlearning}
    \item Experiment details: train two video transformer architectures for 200 epochs on 240K videos of Kinetics-400 which takes 3 days using 64 V100 GPUs.
\end{itemize}

\subsubsection{A large-scale study on unsupervised spatiotemporal representation learning~\cite{DBLP:conf/cvpr/largestudystlearning}}
\begin{itemize}
    \item Evaluate 4 different unsupervised learning frameworks. They find that momentum encoders are more influential than contrastive objectives to finding good representations.
    \item Temporal augmentation: use clips at different temporal locations as positives (improves performance vs. using different spatial crops from a single clip). Using more clips improves performance. It's helpful (or at least not harmful) to sample clips up to a minute apart.
    \item Other types of augmentation: spatial (cropping), color augmentation. Temporal and color have the largest impact on performance, but using all three types leads to the best performance for all frameworks.
    \item For uncurated data, MoCo performs best when using two clips, but BYOL achieves similar performance with four clips
    \item R-50 backbone has significantly better performance than R-18 backbone (+4-9 points), and R-101 backbone has even better performance (+1-2 points). Using more input frames can also help improve performance, but just by a point or two.
\end{itemize}

\subsubsection{Benchmarking representation learning for natural world image collections~\cite{DBLP:conf/cvpr/benchmarkreplearning}}
\begin{itemize}
    \item Two new natural world visual classification datasets, iNat2021 and NeWT (first has 10k species, second is difficult binary classification tasks beyond species class)
    \item Found supervised methods outperformed self-supervised techniques like SimCLR
    \item Find that self-supervised techniques pretrained on ImageNet perform well even on dissimilar datasets of birds (possibly because iNat dataset has birds that aren't the majority of the frame, so different preprocessing may be necessary when using it to pretrain the model)
    \item Self-supervised models struggle on fine-grained classification
    \item Some specific tasks perform better with self-supervised features
    \item Gap between supervised and self-supervised features is larger when trained on iNat vs. Imagenet possibly indicating self—supervised learning techniques are overfit to ImageNet (e.g., hyperparameters/augmentations)
\end{itemize}

\subsection{Active learning}

\subsubsection{A deep active learning system for species identification and counting in camera trap images~\cite{DBLP:journals/corr/alcameratrap,}}
\begin{itemize}
    \item Active learning system to identify and count animals in camera trap images
    \item Pipeline: pre-trained object detection trained on animal class (keep detections with confidence above 90\%); extract 256D embedding from each animal crop using pretrained embedding model; active learning starts with 1k random samples, then each subsequent step picks 100 images to be labeled before retraining
    \item Periodically fine-tune the embedding model on the labeled subset of the target dataset
    \item Tried many active-learning strategies and found K-center strategy has best performance, but all were better than random
\end{itemize}

\subsubsection{LANCET: labeling complex data at scale~\cite{DBLP:journals/pvldb/lancet}}
\begin{itemize}
    \item Automated labeling methods: which objects to ask humans to label? how to automatically propagate labels to other objects? when to stop labeling?
    \item Covariate-shift: idea that in feature space unlabeled object is expected to share the same label with neighbors
    \item Continuity condition: idea that we should pick objects to label while ensuring unlabeled objects always have some sufficiently close labeled neighbors
    \item Key idea: use a distribution matching network to verify whether both covariate-shirt and continuity conditions hold, so it's safe to terminate the labeling process
    \item Raw feature space likely doesn't satisfy covariate-shift condition; propose conditional feature matching (CFM) to learn an embedding that does satisfy it. Add this as a regularization term to the loss function of any embedding method
    \item Feature embedding space depends on classification task
    \item Existing semi-supervised techniques tend to put labeled objects far from decision boundary, so they end up isolated from the unlabeled objects. CFM loss modifies existing semi-supervised techniques so that the feature space satisfies the covariate-shift condition (unlabeled objects must be close to labeled objects if they belong to the same class)
    \item Experiments use SemiGAN with CFM loss to learn feature embedding
    \item Label propagation
    \begin{itemize}
        \item Rather than picking a similarity threshold in feature space, learn a linear model that process a prediction for each unlabeled object
        \item Can be jointly learned with semantic feature extractor
    \end{itemize}
    \item Candidate selection
    \begin{itemize}
        \item Give high priority to unlabeled objects without close labeled neighbors (formalized by Radon-Nikodym derivative, RND)
        \item Exact computation of RND is difficult, so propose to estimate it without first estimating the PDF of labeled and unlabeled data
        \item Use distribution matching network (DMN) that predicts which distribution an object comes from. If distributions are the same, expect error to be around 0.5 because they are indistinguishable
        \item Make training more efficient by using technique of online weight approximation (mini-batches of unlabeled data)
        \item Terminate when weighted distribution of unlabeled objects is similar to distribution of labeled objects (can be checked by DMN), and when RND is bounded by a small value (based on online weight approximation for each unlabeled object)
    \end{itemize}
    \item Experiments
    \begin{itemize}
        \item street view house numbers dataset, cifar-10 dataset, human activity recognition, speech commands
        \item Baselines: Snuba (weak supervised label generation), GOGGLES (images), Core-Set (active learning for DNNs), SemiGAN (ss feature embedding), pretrained AutoEncoder, ground truth
        \item Generated label accuracy: start with random .5\% labeled set
        \item Accuracy of trained models: high accuracy even with a small number of labels
    \end{itemize}
\end{itemize}


\subsubsection{Active learning of an action detector from untrimmed videos~\cite{DBLP:conf/iccv/alactiondetector}}
\begin{itemize}
    \item Input = untrimmed and unlabeled videos; goal is to pick the most useful one for annotation to train action detectors
    \item Challenges: multiple simultaneous actions and extraneous frames belonging to no category of interest (so pooling features may not lead to a good feature descriptor)
    \item Technique highly ranks untrimmed videos with high estimated information content
    \begin{itemize}
        \item Use a Hough-based action detector to estimate spatio-temporal range in which an action of interest could occur
        \item Estimate how each of predicted action intervals would effect action detector if it were labeled (goal is to improve performance across all videos, not just focusing on uncertainty): use an uncertainty metric based on entropy in the 3D vote space of a video
    \end{itemize}
    \item Labeled videos consist of temporal extents of the action in addition to its spatial bounding box in each frame
    \item Detector is based on visual descriptor ``words'' based on HoF and HoG clusterings
    \item Voting procedure of activity detector assumes the time scale of an activity in a new video is comparable to at least one example in the training set
\end{itemize}

\subsubsection{Temporal coherence for active learning in videos~\cite{DBLP:conf/iccvw/altemporalcoherence}}
\begin{itemize}
    \item Target problem: object detection in videos
    \item Approach: temporal coherence. Create nodes in a graph for detections then track them forwards and backwards to link the nodes. Then minimize an energy function on this graphical model
    \item Object detection in videos vs images: temporal coherence between adjacent frames. Therefore active learning strategy focuses on frames with false positives (no support in nearby frames) or false negatives (there is evidence of the object in nearby frames)
    \item Given detections in a frame, use an object tracker to predict its location in preceding/following frames
    \item Assign all detections and candidates ``optimal labels'' using graph cut algorithm, then find the frames with the largest numbers of errors (false positives and/or false negatives)
\end{itemize}

\subsubsection{Leaving some stones unturned: dynamic feature prioritization for activity detection in streaming video~\cite{DBLP:conf/eccv/stonesunturned}}
\begin{itemize}
    \item Learn a policy that dynamically schedules the features to be computed on selected frames of a given test video
    \item Training data: labeled video clips that are temporally clipped
    \item Inference tasks: given a trimmed video, classify the activity; given an untrimmed video, localize a specific activity (binary activity detection)
    \item Step 1: train activity classifier using labeled training data. Features for training are either bag-of-object (given object detectors for object categories, descriptor is likelihood that each object appears in the video clip) or CNN features extracted from each frame. Video descriptors must have temporal locality and be incrementally updatable.
    \item Dynamic feature prioritization is a reinforcement learning problem. The goal is to learn a dynamic policy that maps from partially observed video features to the next most valuable action that will maximize the confidence in the correct prediction.
    \item  Solution is based on a Markov decision process (MDP) that consists of:
    \begin{itemize}
        \item State that captures the history of extracted features and prior actions
        \item Actions the system can perform at each step to extract information from the video. Actions are defined by which information to extract (e.g., which object detector to run) and video location (e.g., which frame to run it on)
        \item Reward for transitioning between states defined in terms of activity recognition. Add a discount term to encourage far-sightedness of selected actions
        \item Policy that picks the next action given the current state to maximize the expected reward
    \end{itemize}
    \item State-action features
    \begin{itemize}
        \item Use training data to learn a linear approximation of $Q^{\pi} = \theta^T \phi(s, a)$. $\phi(s, a)$ is a feature representation of a state-action pair that encodes previous object detection results and the action history which enables the policy to learn useful object co-occurrences and discriminative objects.
        \item $\phi(s_k, a) = [\Psi(X^k), \delta t^k]$ where $\Psi(X^k)$ represents detection results and $\delta t^k$ encodes action history (e.g., how long since each action was performed or binary indicator for whether action was performed).
        \item Learn object co-occurrence: learn a GMM to represent the distribution over the action space using the training data. Use this model to predict the expected values of un-taken actions.
        \item Batch setting: divide video into fixed number of spatio-temporal volumes. This way the number of possible actions (which volume to extract features from) is constant even if videos have different lengths/resolutions.
    \end{itemize}
    \item Reward function measures increase in accuracy across steps. Designed so that actions aren't rewarded for confidence that comes from previous actions.
    \item Dynamic feature prioritization policy: learn the policy using policy iteration. Alternate between learning $\theta$ (which is used to estimate $Q$ given a state-action feature) and generating samples of ${Q^{\pi}(s, a), \phi(s, a)}$. Samples are generated by performing recognition on the training videos.
\end{itemize}

\subsubsection{End-to-end learning of action detection from frame glimpses in videos~\cite{DBLP:conf/cvpr/frameglimpses}}
\begin{itemize}
    \item Input = long, untrimmed video. Output = any instances of a particular action.
    \item Use a recurrent NN architecture to train a policy that picks which video frames to look at next and when to make a prediction
    \item Component 1: Observation network encodes visual representations of frames (where in the video they occur and what they contain)
    \begin{itemize}
        \item Feature vectors of frames are inputs to the recurrent network
        \item Inputs are normalized location ($l_n \in [0, 1]$) and video frame $v_{l_n}$
        \item Architecture: map both $l$ and $v$ to hidden space then combine with fully connected layer (they extract fc7 features from a fine-tuned VGG16 network to map $v$). They use output dimensionality of 1024.
    \end{itemize}
    \item Component 2: Recurrent network sequentially processes frames and decides which frames to look at next and when to make a prediction
    \begin{itemize}
        \item 3 outputs at each step: candidate detection (start, end, confidence); boolean ``should emit'' flag; next frame (can be forward or backwards)
        \item Train the three components using labeled detections in long videos
    \end{itemize}
    \item Implementation
    \begin{itemize}
        \item Learn a 1-vs-all model for each action class. Downsample videos to 1 or 5 fps, then process in sequences of 50 frames where the agent can look at 6 frames/sequence.
        \item Train with minibatches of 256 sequences; they found it was important to tune the number of positive sequences within each minibatch
    \end{itemize}
\end{itemize}

\subsubsection{AdaFrame: adaptive frame selection for fast video recognition~\cite{DBLP:conf/cvpr/adaframe}}
\begin{itemize}
    \item Use a long short-term memory network with global memory
    \item At each time step produce 3 outputs: prediction, which frame to look at next, and the expected reward of looking at more frames
    \item Uniform sampling of frames is inefficient because information isn't uniformly distributed across time
    \item Policy training: reward encourages predictions to be more confident when observing one more frame
    \item Memory-augmented LSTM
    \begin{itemize}
        \item At t-th time step take features of the current frame $v_t$, previous hidden states $h_{t-1}$, cell outputs $c_{t-1}$ and global context vector $u_t$ as inputs and produces current hidden states and cell contents: $h_t, c_t = LSTM([v_t, u_t], h_{t-1}, c_{t-1})$
        \item Hidden states $h_t$ are used as input to a classification prediction network; the probabilities from this network are used to compute reward $r_t$ that measures whether we gained information
        \item Hidden states are also used by selection network to decide where to look next
        \item Hidden states are also used by a utility network to compute the advantage of seeing more frames in the future
    \end{itemize}
    \item Global memory
    \begin{itemize}
        \item Contains a sample of all frames. For each, compute a representation that encodes position and information extracted from a spatial downsampling of the frame
        \item Compute global context information by using the hidden states of the LSTM to find an attention weight for each element in the memory: $z_{t, j} = (W_h h_{t-1})^T PE(v_j^s), \beta_t=softmax(z_t)$ (W transforms hidden states to the correct dimensionality; PE denotes adding position information to features; $\beta_t$ is normalized attention vector over the memory)
        \item Global context vector is the weighted average of the global memory
        \item Intuition is to estimate current progress based on the features in the memory bank
    \end{itemize}
\end{itemize}

\subsection{Data exploration}
\todo{Forager project}
\subsubsection{AIDE: an active learning-based approach for interactive data exploration~\cite{DBLP:journals/tkde/aide}}
\begin{itemize}
    \item Problem setting: use active learning to discover a range query that returns tuples of interest for a user
    \item Iterative exploration model: in each iteration, user marks sample objects as relevant or irrelevant. AIDE generates a model that classifies DB objects as relevant/irrelevant. AIDE uses this model to explore data space further and identify strategic sampling areas
    \item Challenges: accurate results without requiring too many labels and limiting sampling and space exploration overhead
    \item Current active learning approaches don't address challenge of minimizing cost of sample acquisition
    \item AIDE integrates active learning and sample acquisition through exploration heuristics that use classification properties of decision trees to identify promising areas to sample from
    \item Optimizations
    \begin{itemize}
        \item Skew-aware exploration to handle skewed data and interest that lie in sparse/dense parts of distribution
        \item Probabilistic sampling strategy to select most informative sample
        \item Allow user to mark items as relevant, irrelevant or ``similar''
    \end{itemize}
    \item Focus on learning decision tree classifiers because can be easily mapped to queries, and can handle numerical/categorical data
    \item For a given user, divide exploration space into relevant set $T^r$ and irrelevant set $T^{nr}$, which are unknown in advance
    \item Goal: maximize F-measure of final decision tree while minimizing the number of samples presented to user and minimizing the number of extraction queries
    \item Assume user interests are captured by range queries
    \item 3 exploration areas that define sample presented to user in each iteration
    \begin{itemize}
        \item Relevant object discovery: find single relevant objects in yet unexplored areas
        \item Misclassified exploitation: use these relevant objects to generate a model that identifies relevant areas
        \item Boundary exploitation: gradually refine boundaries of relevant areas
    \end{itemize}
    \item Relevant object discovery
    \begin{itemize}
        \item Given exploration on d attributes, create a set of grids that divide space into d-dimensional equip-width cells. Each level has a different granularity
        \item At each level, retrieve one random object from each non-empty cell
    \end{itemize}
    \item Misclassified samples exploitation: increase the number of relevant objects in training set
    \begin{itemize}
        \item False negatives are objects of interest that belong to undiscovered relevant area. AIDE increases set of relevant samples by collecting more objects around false negatives.
        \item Assume that relevant tuples will cluster together, and therefore sapling around FNs will work. Use k-means to generate a sampling area around each cluster of misclassified objects
    \end{itemize}
    \item Boundary exploitation: eliminate irrelevant attributes from the decision tree classifier by domain sampling around the boundaries. Shrink/expand one dimension of a relevant area, and collect samples over the whole domain of the remaining dimensions.
    \item Skew-aware exploration: combine grid with clusters at each level that can better identify dense areas. At each level sample dense areas by collecting one random sample within each cluster at that level, and sample sparse areas by retrieving random samples by grid cells that haven't contributed a sample yet.
    \item Probabilistic sampling: compute posterior probability of a sample x being relevant based on its similarity to existing relevant/irrelevant samples. Present to the user the samples that we are least certain about. Get samples by retrieving all points within a distance $y_i$ from the farthest cluster member in each dimension i.
    \item Similar annotation: use when at least one attribute value is close to a relevant value. Consider samples within some delta. Anticipate the sample from the closer direction will be marked similar/relevant, and sample from wrong direction will be ``irrelevant''
    \item Run exploration on a randomly sampled space that is smaller and therefore more efficient. This works because random sampling maintains the value distribution of the underlying attribute domains.
\end{itemize}


==> response.tex <==
\section*{Response to Reviews}

We thank the reviewers for their insightful feedback.
We addressed the comments as described below.
Significant changes to the original text are highlighted in \revision{}{blue}.

\section*{Meta-Review}

\noindent \textbf{MR-1: Include a more explicit discussion of the novelty over prior labeling approaches (R3.D1) and related work in feature engineering (R3.D2).} \\
\\
\noindent This is an important point. Fundamentally, our contribution does not lie in new ML techniques but in using existing techniques
in a way that produces an interactive, pay-as-you-go system for data exploration in new domains. We added clarifications for both points at the beginning of \Cref{sec:alm} and also in \Cref{subsec:featureselection}. We added a discussion of AutoML to \Cref{sec:relatedwork}. We clarified
that our system supports one type of task: video segment classification at the start of \Cref{sec:alm}. \\



\noindent \textbf{MR-2: Include a conceptual comparison against unsupervised and zero/one/few-shot methods and highlight the advantages and disadvantages of each method (R6.D1). An experimental comparison is not needed if the discussion shows clearly enough that the focus is on a different enough use case.} \\
\\
\noindent We added a discussion of these important points to \Cref{sec:relatedwork}.\\

\noindent \textbf{MR-3: Justify the extra complexity introduced in order to avoid an offline stage (R5.W1).} \\
\\
\noindent We added a justification to \Cref{sec:introduction}. \\


\noindent \textbf{MR-4: Include a more principled discussion of technical details (R5.W2) and justifications (R3.D3 / R3.D4).} \\
\\
\noindent R5.W2: While we used the Anderson-Darling k-sample test (which is nonparametric) to test for uniformity, other statistical tests are possible. We added a description of an alternative test based on the imbalance ratio to \Cref{subsec:activelearning} and show in \Cref{subsec:evalacquisitionfunctionselection} that it performs similarly to the Anderson-Darling-based approach. \\

\noindent R3.D3: To support the claim that active learning approaches often perform no better than random sampling, in addition to the citation,
we now added a forward reference in the introduction to our evaluation section (and figure) where we show that for all but one of the video datasets we evaluated on, neither Coreset sampling nor the more recently-proposed Cluster-Margin sampling performs better than random sampling. \\

\noindent R3.D4: We added additional explanations to \Cref{sec:taskscheduler}.


\noindent \textbf{MR-5: Include a more explicit discussion of potential limitations of this approach like inconsistencies in labeled data, differences in user abilities and experience, and selection of the best representation (R6.D3).} \\
\\
\noindent We added a discussion of \system limitations to \Cref{sec:limitations}.
Additionally, we added results showing \system's robustness to noisy labels to extended technical report~\cite{DBLP:journals/corr/abs-2303-04068}. We omitted them from the paper itself due to space constraints. \\

\noindent \textbf{MR-6: Discuss and then include (if appropriate) in the experiments more recent baselines for active learning approaches (R3.D5/D6).} \\
\\
\noindent  %
We updated \system to use Cluster-Margin sampling when it switches to active learning. We show the updated results in \Cref{sec:evaluation}.
We also looked at the other citation suggested by Reviewer 3 but found that it is intended for a different context. \\


\noindent \textbf{MR-7: Beyond the two video classification datasets, include at least one additional dataset for the same task, or add an additional experimental situation, such as segmentation, detection, and reconstruction.} \\
\\
\noindent Since \system is designed for video classification tasks, we added additional datasets designed to measure video classification performance. Additional results can be found in \Cref{subsec:evalacquisitionfunctionselection} and \Cref{subsec:featureselectioneval}.
\begin{enumerate}
    \item Charades~\cite{DBLP:conf/eccv/SigurdssonVWFLG16}: The task is to determine whether each of 33 verbs occurs in each 30 second video.
    \item Berkeley Deep Drive~\cite{bdd100k}: The task is to determine whether different object types appear in each short video segment (~1.5 seconds).
    \item Bears: A dataset from scientists at UW of primarily nocturnal videos captured from camera traps in Alaska. The task is to determine whether each 5-second video clip contains a bear or not.
    \end{enumerate}

\noindent \textbf{R3.D1: In the active learning manager, the authors wrap random sampling and active learning with a distribution-based discriminator. If the label distribution is skewed, VOCALExplore switches to active learning based sampling. As to the implementation of active learning, they simply adopt an existing method. The contribution is incremental and the novelty of sample selection looks limited.} \\
\\
\noindent See MR-1. \\


\noindent \textbf{R3.D2: The authors incorporate feature selection as part of contributions in active learning manager. I have two concerns for this component. First, the necessity is unclear to me. This part simply belongs to feature engineering in AutoML. If feature selection is an issue for model performance, then I think we also need to determine which type of classification model to use, training set selection (e.g., GLISTER), and hyper-parameter tuning. Second, the generality of this part is questionable. It looks that action recognition is considered in this paper, with 5 pre-defined feature extractors. What happens when the domain experts need to perform other types of video analytical tasks? It looks like we need to re-define the set of feature extractors and re-tune the parameters in the task scheduler.} \\
\\
\noindent See MR-1. \\



\noindent \textbf{R3.D3: The authors use the results in [25] as an evidence to support the claim that “they (active learning approaches) often perform no better than random sampling”. I think it requires careful justification here as the work [25] examines the task of visual question answering, whereas the authors study video frame/segment classification in this paper. The underlying distributions of these two problems may not be the same because the video data tend to be temporally redundant and label skewed.} \\
\\
\noindent See MR-4. \\

\noindent \textbf{R3.D4: The task of scheduler is rule-based and look ad-hoc. In addition, the optimization objective is not explicitly justified. What’s the particular advantage when compared to traditional labeling approaches? From my perspective, the main bottleneck still lies in the amount of efforts paid by the domain experts. If the time of model training becomes an issue, there exist alternative techniques to accelerate this component.} \\
\\
\noindent See MR-4. \\

\noindent \textbf{R3.D5: There are many other active learning approaches to improve the efficacy of sampling. It’s better to incorporate them, especially those published in recent years.} \\
\\
\noindent See MR-6. \\

\noindent \textbf{R3.D6: The baselines used in experimental evaluation are weak. Following D5, it’s better to use more recent works on data sampling.} \\
\\
\noindent See MR-6. \\

\noindent \textbf{R5.W1: A fair amount of complexity is introduced to avoid an offline stage. This part needs more justification.} \\
\\
\noindent See MR-3. \\

\noindent \textbf{R5.W2: Some technical details could be presented in a more principled way.
First, why that test? what assumptions does the test make? Please justify its use.
Second, why that p-value? As you note later in the paper, sample sizes change. The p-value will tend to be smaller for a fixed effect and as the sample grows. Then, why is a pre-specified parameter good enough? This may work for the datasets you tried in the evaluation, but how can we know it'll work for others? I would suggest to either present a principled approach to this, or change the decision criteria. Perhaps moving from p-values to bayes factors or other decision-making boundary that is less sensitive to parameters.} \\
\\
\noindent See MR-4. \\

\noindent \textbf{R5.W2: Other comments/questions:}
\begin{enumerate}
    \item I'd like to see some more details on the data collection (since it's interesting and you have them), how sensitive is VOCALExplore to different video resolutions/quality?
    \begin{itemize}
        \item VOCALExplore is designed to work with any video resolution as we apply a standard short-side scale followed by cropping to generate videos with a uniform resolution before extracting features. The datasets we evaluate on contain videos with resolutions of $568\times320$, $640\times480$, $1280\times720$, and $1920\times1080$. While we expect that videos with low quality will reduce the model performance \system can achieve, it still does quite well on the \bears dataset despite these videos being very noisy. These videos were captured by camera traps at night, so there is poor lighting and a lot of extraneous motion from bugs and rain.
        \item For the \deer dataset specifically, we evaluated on a single day's worth of video for a single deer due to labeling constraints. However, the entire 1.4 TB dataset contains videos from 55 deer.
    \end{itemize}
    \item What are the implications of the statement: ``Note that this algorithm was proposed for the regret minimization setting, while our problem is that of best arm identification (at T points)''
        \begin{itemize}
            \item Although \cite{DBLP:conf/aaai/LiJGSZ020} proposes an algorithm in the ``regret'' minimization setting, the regret is defined in a non-standard manner as a \emph{maximum} over the $T$ interactive iterations rather than as a \emph{summation} (see equation (5) from \cite{DBLP:conf/aaai/LiJGSZ020}). In the classical setting of stationary stochastic bandits, swapping the sum for a max transforms the problem to be very nearly equivalent to best arm identification setting. With this in mind, the relationship between the settings is nuanced and we have clarified the relationship between the settings in \Cref{subsec:featureselection}. \\
        \end{itemize}
      \end{enumerate}

\noindent \textbf{R6.D1: This paper requires users to label data, which is a significant limitation. Although the authors mention that this method is more efficient than similar frameworks, it is not clear whether this process has advantages over unsupervised and zero/one/few-shot methods. Therefore, the authors are advised to make a more detailed comparison with unsupervised and zero/one/few-shot methods and highlight the advantages and disadvantages of each method. \\
}
\\
\noindent See MR-2. \\

\noindent \textbf{R6.D2: This paper only tested its model on two video classification datasets, which may raise questions about whether the model has good generalization ability. Therefore, it is recommended to show results on more tasks, such as segmentation, detection, and reconstruction, to evaluate the effectiveness of the system in different situations and tasks. This can enhance the experimental and reliability of this paper.} \\
\\
\noindent See MR-7. \\

\noindent \textbf{R6.D3: This paper does not discuss the potential limitations or challenges that may arise when using VOCALExplore. These may include inconsistencies in labeled data, differences in user abilities and experience, and selection of the best representation. These potential limitations and challenges should be discussed and addressed to make the VOCALExplore system more reliable and sustainable.} \\
\\
\noindent See MR-5. \\

